On the Robustness of Safe Reinforcement Learning under Observational Perturbations

Safe reinforcement learning (RL) trains a policy to maximize the task reward while satisfying safety constraints. While prior works focus on the performance optimality, we find that the optimal solutions of many safe RL problems are not robust and safe against carefully designed observational perturbations. We formally analyze the unique properties of designing effective observational adversarial attackers in the safe RL setting. We show that baseline adversarial attack techniques for standard RL tasks are not always effective for safe RL and propose two new approaches - one maximizes the cost and the other maximizes the reward. One interesting and counter-intuitive finding is that the maximum reward attack is strong, as it can both induce unsafe behaviors and make the attack stealthy by maintaining the reward. We further propose a robust training framework for safe RL and evaluate it via comprehensive experiments. This paper provides a pioneer work to investigate the safety and robustness of RL under observational attacks for future safe RL studies. Code is available at: \url{https://github.com/liuzuxin/safe-rl-robustness}

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} See Conclusion section.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} See Conclusion section.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
   \answerYes{} See Appendix \ref{app:proof}.
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} See supplementary material.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} See Appendix \ref{app:implementation}.
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} See Appendix \ref{app:implementation}.
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> rebuttal/R1.tex <==

\subsection{Title}
Thanks for the comments, we address the questions as follows.

\subsection{Response}
We thank the reviewer for your time and valuable feedback. We address the concerns as follows.

\textbf{Q1: Stealthiness definition.}
It is an interesting point. 
While most of the RL benchmarks that we know only use lower bounds of the reward to indicate the success of the task, 
we agree that in the real-world applications it is possible that people may get alerted if the result is ''too good to be true''. 
To make our definition more rigorous, we will add constraint to the definition of stealthiness used in this paper as a one-sided stealthiness to the lower bound of the performance. 
We augmented our discussion with a broader definition of stealthiness and provided some examples in the revised Appendix B.1. 
Further exploration on the cognizance to the increase in reward is task-specific and related to human studies, which is set to be future work.


\textbf{Q2: Discussion of two related works.}

Both the Maximum entropy (Eysenbach and Levine, 2022) and WCSAC (Yang et al. 2021) helps enhance the robustness of general RL. However, they lack of key mechanism to improve the robustness against observational adversarial attacks in the CMDP setting, which is one of the major contributions of this paper. We believe this is an important aspect of RL as more and more RL have been deployed to real-world applications.

% Maximum entropy RL (Eysenbach and Levine, 2022) increases the robustness against perturbations on reward function and transition dynamics from a different perspective, i.e., maintaining a diverse stochastic policy. 
% However, it has some limitations towards the safe RL problem. 1) It may not provide a straight-forward way to satisfy the safety constraints requirement of safe RL. 2) It is hard to conduct analysis for observational perturbations.

% WCSAC (Yang et al. 2021) applies the idea of distributional RL to improve safety satisfaction in stochastic environment. WCSAC does improve the robustness against perturbation over transition dynamics. 
% However, they do not consider the robustness w.r.t observational perturbations, which may still lead to successfully adversarial attacks, especially when their distributional policy is close to the safety boundary.

To quantitatively facilitate our analysis, we run the experiments for the maximum-entropy method: SAC-Lagrangian. 
We also run the experiments for another two strong safe RL methods: FOCOPS (suggested by R3) and CVPO (suggested by R4). The detailed results could be found in the revised Appendix C.9. 
The conclusion is that all those methods suffer from the vulnerability issues under the proposed MC and MR attacks, even though they can achieve almost zero constraint violations in noise-free environments.
In addition, the adversarial training (FOCOPS) can help to improve the robustness and safety w.r.t observational adversarial attacks.
Therefore, the maximum-entropy method also struggles to be robust and safe against observational attacks, which also show that the proposed theories and claims in this paper are algorithm-agnostic and could be generalized to different safe RL algorithms.

Nevertheless, we believe that leveraging the information theory and distributional robustness in safe RL is a promising directions. We added a discussion in the last section as our future work. We want to thank the reviewer to raise this point to us.
% utilizing some ideas in the two papers are definitely interesting future directions (e.g., to improve robustness against perturbations over reward function / transition dynamics / policy distribution), but it is out of the scope of this paper. We will add related discussions and references in revision.

\textbf{Q3: On Line 3 of Alg 1: should the state be $\nu(s_0)$?}


It is $\nu(s_t)$ since the attack happens for each time step, so the action at time step $t$ should be sampled from $\pi(\cdot | \nu(s_t))$, where $s_t$ is the state at time step $t$.

\textbf{Q4: On Line 10 of Alg 3 in the appendix: should the samples be based on $\nu$ like on Line 3 of Alg 3?}
Yes, the samples are corrupted ones, we will make it clear in revision.

\textbf{Typo and others.} We thank the reviewer for pointing out the typos and suggestions regarding the presentation. We will revise them accordingly in the final version.

==> rebuttal/R2.tex <==

\subsection{Title}

The natural and straightforward presentation in an under-explored but important area is non-trivial, and is one strength rather than a weakness.

\subsection{Response}
We thank the reviewer for your time and feedback. 

The reviewer's major concern is that proposed method is too ''natural and straightforward''.
However, we humbly cannot agree that a natural and straightforward approach per se weakens the contributions of this paper. 
We believe this work is non-trivial, novel, and beneficial to the research community.
% We believe that insights and novelty in this work is non-trivial which will enrich the research on the analysis of the robustness of safe RL. 
We provide the following facts to support our statement:

1. It is non-trivial and impactful to propose the definitions and results in this work. Though some of them naturally exist in many previous safe RL works, we can rarely see formal discussions of them in the literature.
Bringing those ambiguous, rarely discussed, but important observations together up to the front, organizing and presenting them clearly are a non-negligible contribution in research. 
For instance, the temptation definition together with Lemma 1 can explain why it is hard to find a safe RL methods that can have both highest task reward and the lowest cost, since there are inherent trade-offs for many problems. 
Lemma 2 can explain why the cost curves in many safe RL papers finally converge to the constraint threshold.
Those observations widely exist in the safe RL literature but with limited discussions and formal explanations, and sometimes may even confuse the readers in that "why a method cannot have the highest reward return as well as satisfying the constraints?"
With the definitions and Lemmas we provided, those confusions could be resolved.
We believe using simple ideas to solve an important problem is not worse than proposing a complex method or an obscure theory to solve the same problem.
Furthermore, clearly defining an important and new problem, related definitions, evaluations metrics, and experiment settings for a new area (observational robust safe RL) is by no means a trivial task, but rather requires many intelligence efforts and refinements.
We do believe that our original contributions could improve the awareness of these phenomena and benefit the safe RL community.

2. We provide several insights and novelties in this work. We name a few insights from both theoretical and empirical perspectives as follows:

 - a. The optimal policy in safe RL is vulnerable to observational adversarial attacks (Lemma 1, 2), which is important for safety-critical applications because a non-robust safe policy can hardly be regard as truly safe.
 
 - b. The SOTA attack (MAD, AMAD, minimize reward) and defense (SA-PPOL, adding random noise) methods in standard RL do not work well in the safe RL setting, which means that directly applying them can hardly improve the observational robustness regarding safety.
 
 - c. The proposed maximum reward attack is quite counter-intuitive but performs well. As far as we are aware, we haven't seen any adversarial RL regarding maximizing reward as an attack or even discussing it, which is a key insight and novelty of this paper.
 
 - d. The adversarial training method that underperforms in standard RL setting (Huan et al. 2020) is effective in improving robustness and safety with the proposed MC and MR attackers in safe RL, which is theoretically backed up by Theorem 4, Prop. 2 and 3.
 
 - e. A smoother policy has better robustness (Theorem 2 and 3), which bridges some conclusions in adversarial machine learning with robust safe RL. Also, it is non-trivial to generalize the results in previous work, such as TRPO, to a new problem as the complementary theoretical analysis of the proposed framework, and we haven't seen similar safety performance bounds that consider the smoothness of the policy in the literature.
 
 - f. The experiment results justified most of the claims and proposed insights.
 It is non-trivial to obtain each number in the results of our comprehensive experiments, as each one may take hours or days of computation. We already move more ablation studies in Appendix C.9 but only leave the important ones and give detail analysis in Sec. 5.2. 
 We also provide discussions of the baselines, settings, implementation details, training tricks, and hyperparameters, and explain why baseline doesn't work well in Appendix B and C.
 
It is hard to list all the insights, analysis, and novelties of our work due to the response word limit, but most of them have already been discussed either in the main paper or in the appendix.
As suggested by other reviewers, we also added more ablation results of more safe RL methods (SAC-Lagrangian, FOCOPS, CVPO) at the end of the revised appendix C.9, which show that the major claims and conclusions are generalizable to different methods.

Considering the page limit of the paper, we present a new but important problem in a natural and straightforward way after rounds of polishment, such that the readers can easily capture the main ideas and key messages. 
We believe the easy-to-understand presentation, together with supportive comprehensive experiments and enough insights to an important but rarely discussed area, strengthen our contribution rather than weakening it.
We hope our summary and response could address the reviewer's concern.




% \textbf{Comment 1: The definitions and the results are probability too natural and straightforward.} 
% We agree that many definitions and claims are naturally presented under our carefully polished structure. 
% However, we humbly cannot agree that this straightforward presentation weakens the contribution of this work.
% The reasons are as follows:
% \begin{itemize}
%     \item Though several key definitions and results naturally exist in many previous safe RL works, we can rarely see formal discussions of them. 
%     For instance, the temptation definition together with Lemma 1 can explain why it is hard to make both the reward curves and the cost curves high for a safe RL methods. 
%     Lemma 2 can also explain why the cost curves in many safe RL methods may converge to the constraint threshold.
%     Those observations widely exist in the safe RL literature but with limited discussions and formal explanations, and sometimes may even confuse the readers in that "why a method cannot have the highest reward return as well as satisfying the constraints?"
%     But with the definitions and Lemmas we provided, we can easily address those confusions in the community, and hopefully improve the awareness of them.
%     \item Bringing those ambiguous, rarely discussed, but important phenomenon together up to the front, organizing and presenting them clearly are a non-negligible contribution in our opinion. We do believe that our original contributions could benefit the safe RL community.
    
% \end{itemize}

% \textbf{Comment 2: Hard to see what new insights are gained from the formalization.}

% First, we believe our work provides sufficient insights both from the theoretical side and the empirical side.

% The theoretical analysis serves as complementary materials to support our key arguments, and we believe there are insights from them.
% As we mentioned in Line 210, 217, 218, the insights from Theorem 2 and 3 are that: 1) a smoother policy should be more robust against observational perturbations. This is in line with vast adversarial machine learning literatures [add ref], which bridges the observational robustness in safe RL with them; 2) the adversary's power is restricted by the perturbation range limitation.



% \textbf{Comment 3: The experiment results are not surprising. Move some results to the appendix}

% Our insights from the experiment results are:
% 1) the SOTA adversarial attack and defense methods in standard RL settings may not perform well in the 

% Due to the page limit, we move some discussions to the Appendix section, such as Appendix B, where we discuss the safe RL settings and why SOTA algorithms may not work, and Appendix C.9, where we discussed more experiment results and conduct ablation study. 
% We believe the results on the main content are important to help readers understand the key messages that we want to convey.

==> rebuttal/R3.tex <==

\subsection{Title}
Thanks for the comments.

\subsection{Response}
We appreciate the reviewer for acknowledging this work and the valuable feedback. We address the issues as follows.


\textbf{Q1: Comparison with a recent work.} Thanks for referring this new paper to us. SAAC originally aims to settle the problems of safe exploration and risk-sensitive safety constraint satisfaction. Formally, it trains a policy $\pi_\theta$ by maximizing its discrepancy from the most unsafe policy $\pi_{w^*}$ and the optimization objective is
$$
\max_{\theta} \min_w V_r^{\pi_{\theta}}(\mu_0) - \lambda V_c^{\pi_w}(\mu_0)
$$
where $V_f^{\pi}(\mu_0)$ is the expectation of reward ($f=r$) or cost ($f=c$) value function for initial states under policy $\pi$. While the adversarial training objective in our paper is
$$
\max_{\theta} \min_{\nu} V_r^{\pi\circ\nu}(\mu_0) - \lambda V_c^{\pi\circ\nu}(\mu_0)
$$
where $\pi\circ\nu\doteq \pi(a|\nu(s))$ is the perturbed policy under $\nu$. 

Therefore, SAAC has a similar but slightly different robust optimization objective from us, and it might be hard to ensure the robustness w.r.t observation perturbations. 
But it is indeed an interesting and related algorithm, and we will add related discussions in revision.

% Therefore, SAAC has a robust optimization objective implicitly, which may also defend the observational perturbations (suppose the policy space is smooth w.r.t input state $s$, with small observational perturbation $\nu(s)=s', \|s-s'\|\leq \epsilon$, since $D_{KL}[\pi_\theta(\cdot|s)|\pi_w(\cdot|s)]$ is large, then $D_{KL}[\pi_\theta(\cdot|s')|\pi_w(\cdot|s)]$ is still large, therefore SAAC is robust). However, the robustness of SAAC is too strong for our setting because we only consider the adversaries which only perturb the state $s$ to its neighborhood (e.g., $\nu(s)$ should be in a $\ell_p$-norm ball around $s$). As a result, SAAC may have worse reward performance when maximizing distance to $\pi_{w^*}$. 




\textbf{Q2: Costs may increase and then decease as $\epsilon$ increases.} This is a great question. 
If the perturbation range is large than certain threshold, we can indeed observe that the attack performance may drop.
The intuition in one sentence is that: the neural network-approximated Q functions of reward and cost are not accurate/robust enough to estimate the return correctly around the rollout states/actions and the optimization problem in Eq. (4) could be highly non-convex and non-linear, which can lead to suboptimal solutions of the adversarial perturbations.
In the ideal case, where the Q functions have no prediction errors and the optimization can find the global solution, then the costs should be a monotonic increasing function w.r.t the perturbation range $\epsilon$, but these requirements are hard to be met in practice especially when the perturbation range is large.
For instance, the Q functions may falsely estimate a never-visited state-action-pair's return to be the highest one within the perturbation range, then the attackers is likely to output the suboptimal perturbations that can lead to that state-action-pair.
The effect of the inaccurate Q estimations might be negligible when $\epsilon$ is small, but will be more and more significant as $\epsilon$ increases.
We will add related discussions in the final version and thanks again for pointing out this interesting observation.


\textbf{Q3: FOCOPS experiment.} We thank the reviewer for raising this question. 
First, the proposed claims, such as Lemma 1 and Lemma 2, and the proposed attack and defense methods are independent of the safe RL approaches, since most of them are not intended to robustify the policy network and they may still be close to the safety boundary. 
Therefore, we should observe similar experiment results as the PPO-Lagrangian series.
Second, we conduct the experiments for FOCOPS as requested. We also did robustness evaluation for a maximum-entropy method SAC-Lag (pointed out by R1) and a recent strong safe RL method CVPO (pointed out by R4). The detailed number and results could be found at the end of Appendix C.9.
In summary, all the vanilla safe RL methods -- FOCOPS, SAC-Lag, CVPO -- suffer vulnerability issues under adversarial attacks. That is, though they are safe in noise-free environment, they are not safe anymore under the proposed adversarial attacks.
In addition, the adversarial training can help to improve the robustness and make the FOCOPS agents much safer under strong attacks.
Therefore, the claims and theoretical results in this paper should be generalizable to different safe RL methods, which hopefully can raise more attentions in this field.


\textbf{Q4: p value of the perturbation set.} We mentioned in Line 299-300 that we use $L_{\infty}$ norm for all the experiments, which follows the convention in previous works of robust RL (Huan et al. 2020; 2021). 
We did not try different $p$ values, but it would be an interesting topic to explore in the future.

\textbf{Q5: Maximum reward as a strong attack.} There are multiple reasons of why the MR attack is strong: 1) during training the agent explores enough high-rewarding regions, so the reward Q is well-estimated; 2) the reward signal is dense while the cost signal is sparse and binary, so the reward Q is easier to learn than the cost Q.
The second question is interesting. We believe the "scalar is enough" hypothesis is quite restrictive for many safety-critical applications. It is quite difficult to manually balance the weight between different task objectives as well as the safety constraints. We briefly discuss this in Appendix B.1, and it would be interesting to discuss more along this direction.


\textbf{Q6: Mixed attacks for MC and MR.} 
Technically, it is possible to do so by using a linear combination of the MC and MR as the optimization objective for the adversarial perturbations.
However, we may lose the theoretical properties in Theorem 4, Proposition 2 and 3, and it might be hard to guarantee that which linear weight between them can lead to the best attack performance. 
Empirically, we conduct the experiments following the suggestion by varying the weight between the MR and MC objectives (see revised Appendix C.9), and there is no obvious trend to show which weight performs the best attack. In addition, we believe the performance in practice is heavily dependent on the quality of the learned reward and cost Q functions, as we suggested in Q2. If the reward Q function is learned to be more robust and accurate than the cost Q function, then giving larger weight to the reward Q should achieve better results, and vice versa.


\textbf{Typos.} We thank the reviewer for pointing out the typos, and we will fix them in revision.

==> rebuttal/R4.tex <==
\subsection{Title}
Response to the weakness (Q1) -- clarification of the Bellman equations, Lipschitz assumptions in Theorem 2, 3

\subsection{Response}
We thank the reviewer for your time, valuable feedback, and acknowledgment of our paper's contributions and insights. We address the concerns regarding the theoretical results as follows.

\textbf{Weakness 1, the validity of the Bellman equation of the safe RL case, fixed points, and combined iteration.}

% Zhepeng: I think it's a little wordy, too many sentences may disrupt reviewer. just need to mention 1) policy evaluation is not interconnected; 2) policy improvement is interconnected; 3) Bellman equation is only involved in policy evaluation

Thank you for this insightful question. We provide our explains in two parts: (1) why the Bellman contraction is valid in our analysis; (2) why our presentation Def. 6-8 may have confused you, and how we plan to revise the paper to avoid the misunderstanding.

(1) Similar to most of the safe RL algorithms, such as PPO-Lagrangian, CPO, FOCOPS, LAMBDA, and CVPO, we also consider policy-based (or actor-critic-based) safe RL in this work. 
% First, we are uncertain what does  `combined iteration` mean. 
% We are not considering value-based methods, which are rarely discussed in recent safe RL works, and most deep safe RL methods, such as PPO-Lagrangian, CPO, FOCOPS, LAMBDA, and CVPO, are not value-based, but policy-based or actor-critic-based.
There are two phases for these methods: policy evaluation and policy improvement.
In the \textbf{policy evaluation} phase, the reward and cost value functions $V_r^\pi, V_c^\pi$ are evaluated separately.
At this state, the Bellman operators for reward and cost values are \textit{independent}. Therefore, they have contractions (Def. 6) and will converge to their fixed points separately.
In the \textbf{policy improvement} phase, the interconnections exist since the policy optimizer needs to balance the two value functions together.
However, no Bellman operators are involved in this phase since we directly adopt the reward and cost value in the evaluation phase. 
They are fixed in this stage.
Therefore, we avoid the `combined iteration` for computing the reward and cost values. 
This is a commonly used treatment in safe RL papers to obtain training stability: first evaluating the reward and cost values independently by Bellman equations and then optimizing the policy based on the learned value estimations [refs].

(2) We recheck our writing to see why we misled the reviewer. One thing we can improve is that: perhaps our presentation of the three Bellman operators in Def. 6-8 is too brief (we wanted to save space) thus confusing the reviewer.
The Bellman policy operator in Def. 6 shows that the policy evaluation phase is a contraction for both reward and cost \textit{under observational adversaries}.
The other two operators in Def. 7 and 8 aim to show that finding the optimal adversary that can maximize the reward/cost value given a policy is equivalent to the MR and MC attackers, which are fixed points respectively. 
And they are used to derive the adversarial training properties (Proposition 2 and 3) under the two attackers.
Therefore, when we attack the cost or reward \textbf{separately}, they have the contraction feature, but not when conducted \textbf{together}. 
As a result, we propose the MR and MC approaches separately. 
When they are used simultaneously, we indeed may have the stability issue and lose the contraction property. 
This is the reason why we did not propose a combined approach of MR and MC as inquired by R3. 
We believe because we present the analysis of MR and MC altogether in Theorem 4, we confused the reviewer. 
They should be analyzed and conducted separately. 
But the proposed methods and theoretical analysis are sound, and thus the experiment results do not need to be adjusted. 
We will make the presentation of this part clearer to prevent confusions.

\textbf{Weakness 2, locally Lipschitzness assumption in Theorem 2 and 3.}

We see the reviewer has a concern over the Lipschitz assumption that may prohibit applying the proposed approach in real-world applications.

First, we want to emphasize that the assumption is used in \textit{analysis} rather than \textit{implementation}. Even a policy is not locally Lipschitz, the MC and MR attackers and the adversarial training framework can be implemented. Of course, we will lose the theoretical guarantee of the upper bounds in Theorem 2 and 3.

Second, why do we have to adopt this assumption in the theoretical analysis? Because without the smoothness assumption, the adversary may cause arbitrary cost values, and thus we will lose any guarantee to bound it. For this reason, the Lipschitz assumption is widely adopted in the adversarial machine learning literature, explicitly or implicitly [LOTS of REFS].

Finally, in the real-world application, actions usually take effects via physical \textit{actuators} that are usually continuous. For example, in the automotive case raised by the reviewer, in the real world, bang-bang controller sends signals to the engine or hydraulic braking systems. Their effects on states are continuous with finite Lipschitz constant. Therefore, we think the assumption is valid at least in the fields of robots and automotive. One limitation is that, in some cases, it might be hard to estimate the Lipschitz constant, which is an orthogonal topic of this paper.

Therefore, we believe the Lipschitz is a reasonable assumption and does not prohibit using the proposed method in the real-world application. We hope our response can address the reviewer's concern. 
%We added a discussion of our key assumptions in the Appendix.

% First, we agree that in computer games or a virtual world, the policy could be discrete and non-Lipschitz.
% However, we believe in many real world applications, the `discrete` policy signal will finally be applied to a physical actuator that is continuous (the +1 and -1 signals for mountain car should be applied to continuous physical actuators before running in the real world).
% In that case, the Lipschitz assumption can still be applied w.r.t the physical actuators.

% Second, this is a widely acceptable assumption in theoretical analysis for adversarial machine learning [refs].
% Without the smoothness assumption of the model, people can hardly derive any performance bounds for it. 
% Usually a smoother model means better robustness against input perturbations.
% An infinite Lipschitz constant leads the bound in Theorem 2 and 3 to be infinity, meaning that the adversary may cause arbitrary cost values, which still makes sense.

% Finally, the assumption is only used for theoretical analysis in Theorem 2 and 3 and doesn't affect other findings and results. 
% Even a policy is not locally Lipschitz, as long as Eq. (4) can be solved by any optimization tools, the MC and MR attackers and the adversarial training framework can still work.



\subsection{Title}
Response to Questions 2, 3, and others

\subsection{Response}
We thank the reviewer for raising the questions. We address them as follows.

\textbf{Question 2, more attacks.}

We added discussion of the standard attacks in the RL literature and additional experiments to show the effectiveness of the two approach we proposed.
More specifically, we ... [Add more details what we did. And add numerical results to show the effectiveness of the proposed method.]

As requested, we run the experiments for the minimizing reward attack in for our method, see the updated Appendix for details. It is clear to see that it cannot work in the safe RL setting.
In addition, we adopted one SOTA attack method (MAD) in standard RL as a baseline, and even improve it in the safe RL setting (Line 303-316).
One main conclusion and important finding is that the attacking methods and robust training method in standard RL settings do not perform well in safe RL, which motivates us to propose the MC and MR attackers.
We will make them more clear in the paper.

\textbf{Question 3, no tempting policies.}

As discussed in Line 126, we focus on the discussion of tempting safe RL problems in this paper, because otherwise the safe RL problem is equivalent to a standard RL and is generally considered as a constrained MDP-based safe RL problem. Many algorithms will work well in this case.
We added a discussion in the Appendix for non-tempting settings.


\textbf{More experiments and writing.} We thank the reviewer for the suggestions. We have done the following to improve this paper.

 - We corrected the typos and added a discussion to the references suggested by the reviewer.
 
- We conduct the experiment for the CVPO method (Liu et al. 2022).

- We run the experiments for a maximum entropy-based safe RL method: SAC-Lagrangian (suggested by reviewer 1), and another strong safe RL method: FOCOPS (suggested by reviewer 3).

 - Experiment results show that the vanilla version of them all suffer from vulnerability issues: though they are safe in noise-free environments, they are not safe anymore under strong MC and MR attacks, which again validate that our proposed methods and theories could be applied to a general safe RL setting.
 
- The adversarial training method also successfully makes the FOCOPS method more robust and safe against adversarial attacks, which means that the proposed attack and defense methods are algorithm-agnostic: they can generalize well to different safe RL algorithms.

The detailed results could be found at the end of the revised Appendix C.9.




==> sec4-robust-safe-rl-old.tex <==
\tocless\subsection{Adversarial training against observational perturbations}
\label{sec:adversarial_training}

To defend against observational perturbations, we propose an adversarial safe RL training method.
Similar to adversarial training in the supervised learning literature, we directly optimize the policy upon the attacked sampling trajectories $\Tilde{\tau} = \{s_0, \att_0, s_1, \att_1, ...\}$, where $\att_t \sim \pi(a|\nu(s_t))$.
We can compactly represent the adversarial safe RL objective under observational perturbation as:
\begin{equation}
   \pi^* = \arg\max_{\pi}  V_r^{\pi\circ \nu}(\mu_0), \quad s.t. \quad  V_c^{\pi\circ \nu}(\mu_0) \leq \kappa. %, \quad \nu \in \{\nu_{\text{MC}}, \nu_{\text{MR}}\}
   \label{eq:rsrl_objective}
\end{equation}

The key part is selecting proper adversaries during training to evaluate the value function under observational perturbations accurately, which can be done via the following Bellman operators:

\begin{definition}
Define the Bellman policy operator as $\Tcal_\pi: \sR^{\vert \Scal \vert} \xrightarrow[]{} \sR^{\vert \Scal \vert}$:
\begin{equation}
    (\Tcal_\pi V^{\pi \circ \nu}_f) (s) = \sum_{a\in \Acal} \pi(a|\nu(s)) \sum_{s' \in \Scal} p(s'|s,a) \left[ f(s, a, s') + \gamma V^{\pi \circ \nu}_f (s') \right], \quad f\in \{r, c\}.
\end{equation}
\end{definition}

The Bellman equation can be written as $ V^{\pi \circ \nu}_f (s) = (\Tcal_\pi V^{\pi \circ \nu}_f) (s)$.

\begin{definition}
Define the Bellman adversary effectiveness  operator as $\Tcal_c^*: \sR^{\vert \Scal \vert} \xrightarrow[]{} \sR^{\vert \Scal \vert}$:
\begin{equation}
    (\Tcal_c^* V^{\pi \circ \nu}_c) (s) = \max_{\stt \in B^\epsilon_p(s)} \sum_{a\in \Acal} \pi(a|\stt) \sum_{s' \in \Scal} p(s'|s,a) \left[ c(s, a, s') + \gamma V^{\pi \circ \nu}_c (s') \right].
\end{equation}
\end{definition}

\begin{definition}
Define the Bellman adversary reward stealthiness  operator as $\Tcal_r^*: \sR^{\vert \Scal \vert} \xrightarrow[]{} \sR^{\vert \Scal \vert}$:
\begin{equation}
    (\Tcal_r^* V^{\pi \circ \nu}_r) (s) = \max_{\stt \in B^\epsilon_p(s)} \sum_{a\in \Acal} \pi(a|\stt) \sum_{s' \in \Scal} p(s'|s,a) \left[ r(s, a, s') + \gamma V^{\pi \circ \nu}_r (s') \right].
\end{equation}
\end{definition}
\begin{theorem}[Bellman contraction]
% The Bellman equation can be written as
% $V^{\pi \circ \nu_{\text{MR}}}_r = \Tcal V^{\pi \circ \nu_{\text{MR}}}_r$ for the MR adversary and $V^{\pi \circ \nu_{\text{MC}}}_c = \Tcal V^{\pi \circ \nu_{\text{MC}}}_c$ for the MC adversary.
\revision{Suppose the reward and cost values are estimated independently.}
The Bellman operators $\Tcal_\pi, \Tcal_c^*, \Tcal_r^*$ are contractions under the sup-norm $\Vert \cdot \Vert_\infty$ and will converge to their fixed points, respectively. 
The fixed point for $\Tcal_c^*$ is $V^{\pi \circ \nu_{\text{MC}}}_c = \Tcal_c^{*} V^{\pi \circ \nu_{\text{MC}}}_c$, and the fixed point for $ \Tcal_r^*$ is $V^{\pi \circ \nu_{\text{MR}}}_r = \Tcal_r^* V^{\pi \circ \nu_{\text{MR}}}_r$.
\label{theorem:bellman_contraction}
\end{theorem}

\revision{Independently estimated reward and value functions are implicitly assumed by many safe RL algorithms. We provide detailed explanations of this assumption in Appendix \ref{app:remark_of_safe_rl_setting}.
With this assumption,} Theorem \ref{theorem:bellman_contraction} and \ref{theorem:MCMR} show that we can evaluate the policy performance under one fixed deterministic adversary, which provides the theoretical justification of adversarial training, i.e., training a safe RL agent under observational perturbed sampling trajectories. 
In addition, the value functions under the MC and MR adversaries are the fixed points of the $\Tcal^*_c$ and $\Tcal^*_r$, which suggests that performing adversarial training for the RL agent with the MC \revision{or the} MR attackers will enable the agent to be robust against the most effective \revision{or the} the most reward stealthy perturbations, respectively. 
We have the following propositions:

\begin{proposition}
Suppose an adversarial trained policy $\pi'$ satisfies: $V_c^{\pi' \circ \nu_{\text{MC}}}(\mu_0) \leq \kappa$, then $\pi' \circ \nu$ is guaranteed to be feasible with any $B^\epsilon_p$ bounded adversarial perturbations.
\label{proposition:adv_training_mc}
\end{proposition}

Proposition \ref{proposition:adv_training_mc} indicates that by solving the adversarial constrained optimization problem under the MC attacker, all the feasible solutions will be safe under any bounded adversarial perturbations.

\begin{proposition}
Suppose an adversarial trained policy $\pi'$ satisfies: $V_c^{\pi' \circ \nu_{\text{MR}}}(\mu_0) \leq \kappa$, then $\pi' \circ \nu$ is guaranteed to be non-tempting with any $B^\epsilon_p$ bounded adversarial perturbations.
\label{proposition:adv_training_mr}
\end{proposition}

Proposition \ref{proposition:adv_training_mr} shows a nice property for training a robust policy, since the \texttt{max} operation over the reward in the safe RL objective may lead the policy to the tempting policy class, while the adversarial training with MR attacker can naturally keep the trained policy at safe distance from the tempting policy class.
%, such that the adversarial trained policy will be robust against any bounded reward stealthy attackers.
Practically, we observe that both MC and MR attackers can increase the robustness and safety via adversarial training, and could be easily plugged into any safe RL algorithms, in principle.

\vspace{-3mm}
\tocless\subsection{Practical implementation}
\vspace{-2mm}

The meta adversarial training algorithm is shown in Algo. \ref{algo:meta-algorithm}.
We particularly adopt the primal-dual methods~\citep{ray2019benchmarking, stooke2020responsive, tessler2018reward} that are widely used in the safe RL literature as the \texttt{learner}, then the adversarial training objective in Eq. (\ref{eq:rsrl_objective}) can be converted to a min-max form by using the Lagrange multiplier $\lambda$:

\vspace{-3mm}
\begin{equation}
   (\pi^*, \lambda^*) = \min_{\lambda\geq0}\max_{\pi\in \Pi} V_r^{\pi\circ \nu}(\mu_0) - \lambda ( V_c^{\pi\circ \nu}(\mu_0) - \kappa) %, \quad \nu \in \{\nu_{\text{MC}}, \nu_{\text{MR}}\}
   \label{eq:lagrangian}
\end{equation}
\vspace{-4mm}

Solving the inner maximization (primal update) via any policy optimization methods and the outer minimization (dual update) via gradient descent iteratively yields the Lagrangian algorithm.
Under proper learning rates and bounded noise assumptions, the iterates ($\pi_n, \lambda_n$) converge to a fixed point (a local minimum) almost surely~\citep{tessler2018reward,paternain2019constrained}.
We will particularly use PPO \citep{schulman2017proximal} in the primal update.

\begin{wrapfigure}{R}{0.65\textwidth}
\begin{minipage}{0.64\textwidth}
\vspace*{-0.15in}
\begin{algorithm}[H]
\caption{Adversarial safe RL training meta algorithm}
{\bfseries Input:} Policy class $\Pi$, Safe RL \texttt{learner}, Adversary \texttt{scheduler} \par
{\bfseries Output:} \raggedright Observational robust policy $\pi$ \par
\begin{algorithmic}[1] % The number tells where the line numbering should start
\STATE Initialize policy $\pi \in \Pi$ and adversary $\nu :\Scal \xrightarrow{} \Scal$
\FOR{each training epoch $n=1,..., N$}
\STATE Rollout trajectories: $\Tilde{\tau} = \{s_0, \att_0, ...\}_T$, $\att_t \sim \pi(a|\nu(s_t))$
\STATE Run safe RL learner: $\pi \xleftarrow{} \texttt{learner}(\Tilde{\tau}, \Pi)$

\STATE Update adversary: $\nu \xleftarrow{} \texttt{scheduler}(\Tilde{\tau}, \pi, n)$

\ENDFOR
\end{algorithmic}
\label{algo:meta-algorithm}
\end{algorithm}
\end{minipage}
\vspace*{-0.1in}
\end{wrapfigure}


Based on previous theoretical analysis, we adopt MC or MR as the adversary when sampling trajectories.
The \texttt{scheduler} function aims to train the reward and cost Q-value functions for the MR and the MC attackers, because many on-policy algorithms such as PPO do not provide them.
In addition, the scheduler can update the power of the adversary based on the learning progress accordingly, since a strong adversary at the beginning may prohibit the \texttt{learner} from exploring the environment and thus corrupt the training.
We gradually increase the perturbation range $\epsilon$ along with the training epochs to adjust the adversary perturbation set $B^\epsilon_p$, such that the agent will not be too conservative in the early stage of training.
A similar idea is also used in adversarial training literature~\citep{salimans2016improved, arjovsky2017towards,gowal2018effectiveness} and the curriculum learning literature \citep{dennis2020emergent, portelas2020automatic}.
See more implementation details in Appendix \ref{app:adversarial_training_impl}. 
